On the supersingular K3 surface in characteristic 5 with Artin invariant 1

We present three interesting projective models of the supersingular K3 surface X in characteristic 5 with Artin invariant 1. For each projective model, we determine smooth rational curves on X with the minimal degree and the projective automorphism group. Moreover, by using the superspecial abelian surface, we construct six sets of 16 disjoint smooth rational curves on X, and show that they form a beautiful configuration.

==> FSF25.tex <==
$$
\begin{array}{lll}
 P_{1}:=[0: 1: 2] & 
 P_{2}:=[0: 1: 3] & 
 P_{3}:=[0: 1: 1+\sqrttwo]\\
 P_{4}:=[0: 1: 4+\sqrttwo] & 
 P_{5}:=[0: 1: 1+4\sqrttwo] & 
 P_{6}:=[0: 1: 4+4\sqrttwo]\\
 P_{7}:=[1: 0: 2] & 
 P_{8}:=[1: 0: 3] & 
 P_{9}:=[1: 0: 1+\sqrttwo]\\
 P_{10}:=[1: 0: 4+\sqrttwo] & 
 P_{11}:=[1: 0: 1+4\sqrttwo] & 
 P_{12}:=[1: 0: 4+4\sqrttwo]\\
 P_{13}:=[1: 1: \sqrttwo] & 
 P_{14}:=[1: 1: 1+2\sqrttwo] & 
 P_{15}:=[1: 1: 4+2\sqrttwo]\\
 P_{16}:=[1: 1: 1+3\sqrttwo] & 
 P_{17}:=[1: 1: 4+3\sqrttwo] & 
 P_{18}:=[1: 1: 4\sqrttwo]\\
 P_{19}:=[1: 2: 0] & 
 P_{20}:=[1: 3: 0] & 
 P_{21}:=[1: 4: \sqrttwo]\\
 P_{22}:=[1: 4: 1+2\sqrttwo] & 
 P_{23}:=[1: 4: 4+2\sqrttwo] & 
 P_{24}:=[1: 4: 1+3\sqrttwo]\\
 P_{25}:=[1: 4: 4+3\sqrttwo] & 
 P_{26}:=[1: 4: 4\sqrttwo] & 
 P_{27}:=[1: \sqrttwo: 1]\\
 P_{28}:=[1: \sqrttwo: 4] & 
 P_{29}:=[1: \sqrttwo: 2+2\sqrttwo] & 
 P_{30}:=[1: \sqrttwo: 3+2\sqrttwo]\\
 P_{31}:=[1: \sqrttwo: 2+3\sqrttwo] & 
 P_{32}:=[1: \sqrttwo: 3+3\sqrttwo] & 
 P_{33}:=[1: 1+\sqrttwo: 0]\\
 P_{34}:=[1: 2+\sqrttwo: 2+\sqrttwo] & 
 P_{35}:=[1: 2+\sqrttwo: 3+\sqrttwo] & 
 P_{36}:=[1: 2+\sqrttwo: 2\sqrttwo]\\
 P_{37}:=[1: 2+\sqrttwo: 3\sqrttwo] & 
 P_{38}:=[1: 2+\sqrttwo: 2+4\sqrttwo] & 
 P_{39}:=[1: 2+\sqrttwo: 3+4\sqrttwo]\\
 P_{40}:=[1: 3+\sqrttwo: 2+\sqrttwo] & 
 P_{41}:=[1: 3+\sqrttwo: 3+\sqrttwo] & 
 P_{42}:=[1: 3+\sqrttwo: 2\sqrttwo]\\
 P_{43}:=[1: 3+\sqrttwo: 3\sqrttwo] & 
 P_{44}:=[1: 3+\sqrttwo: 2+4\sqrttwo] & 
 P_{45}:=[1: 3+\sqrttwo: 3+4\sqrttwo]\\
 P_{46}:=[1: 4+\sqrttwo: 0] & 
 P_{47}:=[1: 2\sqrttwo: 2+\sqrttwo] & 
 P_{48}:=[1: 2\sqrttwo: 3+\sqrttwo]\\
 P_{49}:=[1: 2\sqrttwo: 2\sqrttwo] & 
 P_{50}:=[1: 2\sqrttwo: 3\sqrttwo] & 
 P_{51}:=[1: 2\sqrttwo: 2+4\sqrttwo]\\
 P_{52}:=[1: 2\sqrttwo: 3+4\sqrttwo] & 
 P_{53}:=[1: 1+2\sqrttwo: 1] & 
 P_{54}:=[1: 1+2\sqrttwo: 4]\\
 P_{55}:=[1: 1+2\sqrttwo: 2+2\sqrttwo] & 
 P_{56}:=[1: 1+2\sqrttwo: 3+2\sqrttwo] & 
 P_{57}:=[1: 1+2\sqrttwo: 2+3\sqrttwo]\\
 P_{58}:=[1: 1+2\sqrttwo: 3+3\sqrttwo] & 
 P_{59}:=[1: 2+2\sqrttwo: \sqrttwo] & 
 P_{60}:=[1: 2+2\sqrttwo: 1+2\sqrttwo]\\
 P_{61}:=[1: 2+2\sqrttwo: 4+2\sqrttwo] & 
 P_{62}:=[1: 2+2\sqrttwo: 1+3\sqrttwo] & 
 P_{63}:=[1: 2+2\sqrttwo: 4+3\sqrttwo]\\
 P_{64}:=[1: 2+2\sqrttwo: 4\sqrttwo] & 
 P_{65}:=[1: 3+2\sqrttwo: \sqrttwo] & 
 P_{66}:=[1: 3+2\sqrttwo: 1+2\sqrttwo]\\
 P_{67}:=[1: 3+2\sqrttwo: 4+2\sqrttwo] & 
 P_{68}:=[1: 3+2\sqrttwo: 1+3\sqrttwo] & 
 P_{69}:=[1: 3+2\sqrttwo: 4+3\sqrttwo]\\
 P_{70}:=[1: 3+2\sqrttwo: 4\sqrttwo] & 
 P_{71}:=[1: 4+2\sqrttwo: 1] & 
 P_{72}:=[1: 4+2\sqrttwo: 4]\\
 P_{73}:=[1: 4+2\sqrttwo: 2+2\sqrttwo] & 
 P_{74}:=[1: 4+2\sqrttwo: 3+2\sqrttwo] & 
 P_{75}:=[1: 4+2\sqrttwo: 2+3\sqrttwo]\\
 P_{76}:=[1: 4+2\sqrttwo: 3+3\sqrttwo] & 
 P_{77}:=[1: 3\sqrttwo: 2+\sqrttwo] & 
 P_{78}:=[1: 3\sqrttwo: 3+\sqrttwo]\\
 P_{79}:=[1: 3\sqrttwo: 2\sqrttwo] & 
 P_{80}:=[1: 3\sqrttwo: 3\sqrttwo] & 
 P_{81}:=[1: 3\sqrttwo: 2+4\sqrttwo]\\
 P_{82}:=[1: 3\sqrttwo: 3+4\sqrttwo] & 
 P_{83}:=[1: 1+3\sqrttwo: 1] & 
 P_{84}:=[1: 1+3\sqrttwo: 4]\\
 P_{85}:=[1: 1+3\sqrttwo: 2+2\sqrttwo] & 
 P_{86}:=[1: 1+3\sqrttwo: 3+2\sqrttwo] & 
 P_{87}:=[1: 1+3\sqrttwo: 2+3\sqrttwo]\\
 P_{88}:=[1: 1+3\sqrttwo: 3+3\sqrttwo] & 
 P_{89}:=[1: 2+3\sqrttwo: \sqrttwo] & 
 P_{90}:=[1: 2+3\sqrttwo: 1+2\sqrttwo]\\
 P_{91}:=[1: 2+3\sqrttwo: 4+2\sqrttwo] & 
 P_{92}:=[1: 2+3\sqrttwo: 1+3\sqrttwo] & 
 P_{93}:=[1: 2+3\sqrttwo: 4+3\sqrttwo]\\
 P_{94}:=[1: 2+3\sqrttwo: 4\sqrttwo] & 
 P_{95}:=[1: 3+3\sqrttwo: \sqrttwo] & 
 P_{96}:=[1: 3+3\sqrttwo: 1+2\sqrttwo]\\
 P_{97}:=[1: 3+3\sqrttwo: 4+2\sqrttwo] & 
 P_{98}:=[1: 3+3\sqrttwo: 1+3\sqrttwo] & 
 P_{99}:=[1: 3+3\sqrttwo: 4+3\sqrttwo]\\
 P_{100}:=[1: 3+3\sqrttwo: 4\sqrttwo] & 
 P_{101}:=[1: 4+3\sqrttwo: 1] & 
 P_{102}:=[1: 4+3\sqrttwo: 4]\\
 P_{103}:=[1: 4+3\sqrttwo: 2+2\sqrttwo] & 
 P_{104}:=[1: 4+3\sqrttwo: 3+2\sqrttwo] & 
 P_{105}:=[1: 4+3\sqrttwo: 2+3\sqrttwo]\\
 P_{106}:=[1: 4+3\sqrttwo: 3+3\sqrttwo] & 
 P_{107}:=[1: 4\sqrttwo: 1] & 
 P_{108}:=[1: 4\sqrttwo: 4]\\
 P_{109}:=[1: 4\sqrttwo: 2+2\sqrttwo] & 
 P_{110}:=[1: 4\sqrttwo: 3+2\sqrttwo] & 
 P_{111}:=[1: 4\sqrttwo: 2+3\sqrttwo]\\
 P_{112}:=[1: 4\sqrttwo: 3+3\sqrttwo] & 
 P_{113}:=[1: 1+4\sqrttwo: 0] & 
 P_{114}:=[1: 2+4\sqrttwo: 2+\sqrttwo]\\
 P_{115}:=[1: 2+4\sqrttwo: 3+\sqrttwo] & 
 P_{116}:=[1: 2+4\sqrttwo: 2\sqrttwo] & 
 P_{117}:=[1: 2+4\sqrttwo: 3\sqrttwo]\\
 P_{118}:=[1: 2+4\sqrttwo: 2+4\sqrttwo] & 
 P_{119}:=[1: 2+4\sqrttwo: 3+4\sqrttwo] & 
 P_{120}:=[1: 3+4\sqrttwo: 2+\sqrttwo]\\
 P_{121}:=[1: 3+4\sqrttwo: 3+\sqrttwo] & 
 P_{122}:=[1: 3+4\sqrttwo: 2\sqrttwo] & 
 P_{123}:=[1: 3+4\sqrttwo: 3\sqrttwo]\\
 P_{124}:=[1: 3+4\sqrttwo: 2+4\sqrttwo] & 
 P_{125}:=[1: 3+4\sqrttwo: 3+4\sqrttwo] & 
 P_{126}:=[1: 4+4\sqrttwo: 0]\\
\end{array}
$$


==> Flip.tex <==
\left[ \begin {array}{cccccccccccccccccccccc} 0\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\\
\nalmed 1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1
\end {array} \right] 

==> Frconjmatdual.tex <==
\left[ \begin {array}{cccccccccccccccccccccc}
1\shrnk &0\shrnk &0\shrnk &0\shrnk &2\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nnalmed
0\shrnk &1\shrnk &0\shrnk &0\shrnk &3\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nnalmed
0\shrnk &0\shrnk &1\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &0\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &1\shrnk &0\shrnk &0\shrnk &1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &-1\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &1\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &-1\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-2\shrnk &1\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &0\shrnk &0\shrnk &1\shrnk &0\shrnk &1\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &0\shrnk &0\shrnk &1\shrnk &0\shrnk &0\shrnk &1\shrnk &0\shrnk &0\shrnk &1\shrnk &0\shrnk &1\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &-1\shrnk &1\shrnk &-1\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &0\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &0\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &1\shrnk &0\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &1\shrnk &-1\shrnk &1\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &1\shrnk &1\shrnk &0\shrnk &0\shrnk &0\shrnk &1\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\shrnk &0\\
\nnalmed
0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &0\shrnk &-1\end {array} \right] 


==> newD.tex <==
We say that an induced chambers $D$ and $D\sprime$ are  \emph{$G_X$-congruent} 
 if there exists $g\in G_X$
such that $D^g=D\sprime$.
The number of $G_X$-conguence classes is finite. 
To determine the automorphism group of $X$ by the generalized Borcherds method decribed in~\cite{},
we need to obtain the list of all $G_X$-conguence classes.
Let $D$ be an induced chamber.
We define the \emph{level} of $D$ to be the minimal non-negative integer $\ell$ such that
there exists a chain
$$
D^{(0)}=D_0, D^{(1)}, \dots, D^{(\ell)}=D
$$ of induced chambers such that $D^{(i-1)}$ and $D^{(i)}$ are adjacent.
We have made the list of the $G_X$-conguence classes of  induced chambers of level$< 4$.
The number is
$$
\begin{array}{cc}
\text{level} & \text{number of $G_X$-conguence classes}\\
0 & 1 \\
1 & 2\\
2 & 12\\
3 & 328
\end{array}
$$
For level $4$, we have found more than $6000$ $G_X$-conguence classes,
and we have given up the computation.
The data of the  induced chambers $D$ of level $2$ is as follows.
The first column is the order of $\Aut_X(D)$.
The second column is the orbit decomposition of the $(-2)$-walls of $D$ by the action of \Aut_X(D)$.
$$
\begin{array}{cc}
 360& [18, 60]\\
36& [6, 9, 18, 18]\\
36& [6, 9, 18, 18]\\
48& [6, 8, 12, 24]\\
48& [6, 8, 12, 24]\\
72& [3, 12, 12, 18]\\
12& [3, 6, 6, 6, 6, 12]\\
8& [2, 2, 2, 4, 4, 4, 4, 4, 8, 8]\\
2& [1, 1, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2]\\
6& [2, 2, 3, 3, 3, 3, 6, 6, 6]\\
6& [2, 2, 3, 3, 3, 3, 6, 6, 6]\\
8& [2, 4, 4, 4, 4, 8, 8]
\end{array}
$$




==> orbitdecomptable0.tex <==
%nowver/orbitdecomptable0.tex
&&
\begin{array}{l|cccccc}
\textrm{no. }&0 &1 &2 & &  & \\
\cline{1-6}
\textrm{cardinality}&252 &300 &15750 & &  & \\
\textrm{type}&[1,-2]&[1,-8/5]&[2,-6/5]& &  & \end{array}


==> orbitdecomptable1.tex <==
%nowver/orbitdecomptable1.tex
&&
\begin{array}{l|cccccc}
\textrm{no. }& 0 &1 &2 &3 &4 &\\
\cline{1-6}
\textrm{cardinality}&168 &8 &15 &15 &70 &\\
\textrm{type}&[1,-2]&[3/5,-8/5]&[4/5,-8/5]&[4/5,-8/5]&[6/5,-8/5]&\end{array}
\\
&&
\begin{array}{l|cccccc}
\textrm{no. }&5  &6 &7 &8 &9 &\\
\cline{1-6}
\textrm{cardinality}&70 &168 &280 &280 &840 &\\
\textrm{type}&[6/5,-8/5]&[7/5,-8/5]&[9/5,-6/5]&[9/5,-6/5]&[2,-6/5]&\end{array}
\\
&&
\begin{array}{l|cccccc}
\textrm{no. }&10  &11 &12 &13 &14 &\\
\cline{1-6}
\textrm{cardinality}&840 &1680 &1680 &840 &840 &\\
\textrm{type}&[2,-6/5]&[11/5,-6/5]&[11/5,-6/5]&[11/5,-6/5]&[11/5,-6/5]&\end{array}
\\
&&
\begin{array}{l|cccccc}
\textrm{no. }&15 &16 &17 & & &   \\
\cline{1-6}
\textrm{cardinality}&15 &15 &8 & &  & \\
\textrm{type}&[8/5,-4/5]&[8/5,-4/5]&[9/5,-2/5]& &  & \end{array}


==> orbitdecomptable2.tex <==
%nowver/orbitdecomptable2.tex
&&
\begin{array}{l|cccccc}
\textrm{no. }& 0&1 &2 &3 &4  &\\
\cline{1-6}
\textrm{cardinality}&48 &48 &4 &4 &16 &\\
\textrm{type}&[1,-2]&[1,-2]&[2/5,-8/5]&[2/5,-8/5]&[1,-8/5]&\end{array}
\\
&&
\begin{array}{l|cccccc}
\textrm{no. }&5 &6 &7 &8 &9  &\\
\cline{1-6}
\textrm{cardinality}&16 &64 &72 &64 &72 &\\
\textrm{type}&[1,-8/5]&[8/5,-8/5]&[8/5,-8/5]&[8/5,-8/5]&[8/5,-8/5]&\end{array}
\\
&&
\begin{array}{l|cccccc}
\textrm{no. }&10 &11 &12 &13 &14  &\\
\cline{1-6}
\textrm{cardinality}&24 &16 &48 &48 &16 &\\
\textrm{type}&[8/5,-6/5]&[9/5,-6/5]&[9/5,-6/5]&[9/5,-6/5]&[9/5,-6/5]&\end{array}
\\
&&
\begin{array}{l|cccccc}
\textrm{no. }&15 &16 &17 &18 &19  &\\
\cline{1-6}
\textrm{cardinality}&48 &96 &288 &288 &96 &\\
\textrm{type}&[11/5,-6/5]&[11/5,-6/5]&[11/5,-6/5]&[11/5,-6/5]&[11/5,-6/5]&\end{array}
\\
&&
\begin{array}{l|cccccc}
\textrm{no. }&20 &21 &22 &23 &24  &\\
\cline{1-6}
\textrm{cardinality}&48 &576 &192 &192 &144 &\\
\textrm{type}&[11/5,-6/5]&[12/5,-6/5]&[12/5,-6/5]&[12/5,-6/5]&[12/5,-6/5]&\end{array}
\\
&&
\begin{array}{l|cccccc}
\textrm{no. }&25 &26 & &  &   \\
\cline{1-6}
\textrm{cardinality}&3 &3 & &  &  & \\
\textrm{type}&[8/5,-4/5]&[8/5,-4/5]& &  &  & \end{array}

